Lattice Green's functions for Poisson problems with two unbounded and one periodic direction

Fourier-based Poisson solvers treat periodic directions spectrally and unbounded ones by the Hockney--Eastwood convolution with a free-space kernel. With two unbounded and one periodic direction, the setting of vortex tubes, wakes and jets, the kernel used so far by these solvers combines the two-dimensional kernel on the zero periodic mode with the symbol of the operator sampled on the doubled grid on every other mode. We show that the second ingredient is not exact: the error is the field of the periodic images of the source and independent of the mesh size. While the period $L_z$ is not much longer than the unbounded extent $L_x$, it is of order $\exp(-2\pi d/L_z)$, with $d$ the distance to the nearest image; beyond, it grows like $(L_z/L_x)^2$. The error is thus small on cubic domains, but larger than the solution itself on elongated ones. We remove the approximation by extending the integral representation of the exact second-order kernel of Hou and Colonius: the screened kernel of each mode is evaluated in closed form along one unbounded direction and by Gauss--Legendre quadrature along the other, for the high-order dimension-split and Mehrstellen stencils, at a one-off cost of about one solve. The kernels, implemented in the open-source library \flups{}, are verified by comparison with independent quadratures, by a padding test sensitive to the boundary condition enforced, and by convergence at the order of each stencil on an axially modulated tube source, on domains up to $64$ times longer than wide and up to $2.7\times10^{11}$ unknowns.

==> data/images_sketch/Lz16_err.tex <==
% generated by gen_images_sketch.py: Lz/Lx=16, x/Lx, y = value/2.7*0.95
\def\sketchcurve{plot coordinates {(0.0000,0.85633)(0.2450,0.84999)(0.5000,0.84784)(0.7550,0.84999)(1.0000,0.85633)}}%


==> data/images_sketch/Lz16_free.tex <==
% generated by gen_images_sketch.py: Lz/Lx=16, x/Lx, y = value/2.7*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.04190)(-1.4600,0.05905)(-1.2050,0.06915)(-0.9750,0.08029)(-0.7650,0.09271)(-0.5750,0.10646)(-0.4050,0.12155)(-0.2550,0.13793)(-0.1350,0.15394)(-0.0250,0.17187)(0.0700,0.19097)(0.1550,0.21230)(0.2250,0.23446)(0.2850,0.25866)(0.3250,0.27899)(0.3950,0.32046)(0.4300,0.33727)(0.4650,0.34812)(0.5000,0.35185)(0.5300,0.34910)(0.5650,0.33922)(0.6000,0.32316)(0.6800,0.27621)(0.7300,0.25202)(0.8050,0.22432)(0.8950,0.19917)(1.0050,0.17557)(1.1350,0.15394)(1.2850,0.13437)(1.4550,0.11678)(1.6650,0.09960)(1.9000,0.08444)(2.1700,0.07071)(2.4700,0.05870)(2.8050,0.04816)(3.1750,0.03908)(4.0500,0.02449)}}%


==> data/images_sketch/Lz16_imgm1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=16, x/Lx, y = value/2.7*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.16746)(-1.9750,0.18142)(-1.9100,0.19557)(-1.8500,0.21090)(-1.7950,0.22758)(-1.7450,0.24580)(-1.7050,0.26336)(-1.6700,0.28184)(-1.6050,0.32046)(-1.5700,0.33727)(-1.5500,0.34429)(-1.5300,0.34910)(-1.4950,0.35178)(-1.4600,0.34698)(-1.4250,0.33520)(-1.3900,0.31769)(-1.3050,0.26830)(-1.2700,0.25202)(-1.2300,0.23626)(-1.1850,0.22117)(-1.1350,0.20682)(-1.0200,0.18042)(-0.9450,0.16660)(-0.8600,0.15321)(-0.6700,0.12931)(-0.4450,0.10808)(-0.1800,0.08921)(0.1350,0.07231)(0.5000,0.05764)(0.9150,0.04522)(1.3850,0.03482)(1.9200,0.02620)(2.5300,0.01916)(4.0500,0.00912)}}%


==> data/images_sketch/Lz16_imgp1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=16, x/Lx, y = value/2.7*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.01479)(-1.4200,0.02026)(-0.8650,0.02696)(-0.3750,0.03501)(0.0600,0.04458)(0.4450,0.05577)(0.7900,0.06893)(1.0900,0.08387)(1.3550,0.10107)(1.5700,0.11913)(1.7600,0.13977)(1.9250,0.16326)(2.0600,0.18876)(2.1550,0.21230)(2.2350,0.23809)(2.2700,0.25202)(2.3050,0.26830)(2.3900,0.31769)(2.4250,0.33520)(2.4450,0.34274)(2.4650,0.34812)(2.5000,0.35185)(2.5350,0.34812)(2.5550,0.34274)(2.5750,0.33520)(2.6100,0.31769)(2.6700,0.28184)(2.7000,0.26580)(2.7400,0.24783)(2.7900,0.22925)(2.8400,0.21372)(2.9000,0.19795)(2.9650,0.18346)(3.0350,0.17008)(3.1250,0.15543)(3.2250,0.14165)(3.4550,0.11678)(3.7300,0.09504)(4.0500,0.07641)}}%


==> data/images_sketch/Lz1_err.tex <==
% generated by gen_images_sketch.py: Lz/Lx=1, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(0.0000,0.00004)(1.0000,0.00004)}}%


==> data/images_sketch/Lz1_free.tex <==
% generated by gen_images_sketch.py: Lz/Lx=1, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.00000)(-0.6850,0.00028)(-0.3250,0.00317)(-0.1900,0.00807)(-0.0900,0.01629)(-0.0100,0.02883)(0.0250,0.03714)(0.0550,0.04624)(0.0900,0.05984)(0.1200,0.07484)(0.1500,0.09385)(0.1750,0.11361)(0.2000,0.13787)(0.2200,0.16129)(0.2400,0.18910)(0.2600,0.22224)(0.2900,0.28472)(0.3050,0.32322)(0.3200,0.36779)(0.3400,0.43742)(0.4000,0.66957)(0.4300,0.76478)(0.4500,0.81236)(0.4650,0.83830)(0.4750,0.85066)(0.4850,0.85895)(0.5000,0.86364)(0.5150,0.85895)(0.5250,0.85066)(0.5350,0.83830)(0.5500,0.81236)(0.5700,0.76478)(0.6000,0.66957)(0.6600,0.43742)(0.6800,0.36779)(0.6950,0.32322)(0.7100,0.28472)(0.7250,0.25132)(0.7450,0.21339)(0.7650,0.18169)(0.7900,0.14908)(0.8150,0.12271)(0.8450,0.09749)(0.8750,0.07771)(0.9100,0.05984)(0.9500,0.04457)(0.9900,0.03332)(1.0650,0.01945)(1.1550,0.01030)(1.2700,0.00463)(1.4250,0.00160)(1.8500,0.00009)(4.0500,0.00000)}}%


==> data/images_sketch/Lz1_imgm1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=1, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.02164)(-1.9950,0.03213)(-1.9500,0.04457)(-1.9100,0.05984)(-1.8750,0.07771)(-1.8400,0.10128)(-1.8100,0.12756)(-1.7850,0.15506)(-1.7600,0.18910)(-1.7400,0.22224)(-1.7200,0.26194)(-1.7000,0.30977)(-1.6850,0.35220)(-1.6600,0.43742)(-1.6000,0.66957)(-1.5800,0.73592)(-1.5650,0.77799)(-1.5450,0.82197)(-1.5300,0.84498)(-1.5150,0.85895)(-1.5000,0.86364)(-1.4850,0.85895)(-1.4700,0.84498)(-1.4550,0.82197)(-1.4350,0.77799)(-1.4200,0.73592)(-1.4000,0.66957)(-1.3400,0.43742)(-1.3150,0.35220)(-1.3000,0.30977)(-1.2800,0.26194)(-1.2600,0.22224)(-1.2400,0.18910)(-1.2150,0.15506)(-1.1900,0.12756)(-1.1600,0.10128)(-1.1250,0.07771)(-1.0900,0.05984)(-1.0500,0.04457)(-1.0050,0.03213)(-0.9500,0.02164)(-0.8700,0.01228)(-0.7650,0.00590)(-0.6300,0.00233)(-0.4400,0.00064)(4.0500,0.00000)}}%


==> data/images_sketch/Lz1_imgp1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=1, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.00000)(1.5050,0.00100)(1.6800,0.00328)(1.8050,0.00779)(1.9000,0.01517)(1.9800,0.02683)(2.0250,0.03714)(2.0650,0.04976)(2.1000,0.06446)(2.1350,0.08378)(2.1650,0.10522)(2.1950,0.13260)(2.2200,0.16129)(2.2450,0.19684)(2.2650,0.23150)(2.2800,0.26194)(2.3000,0.30977)(2.3150,0.35220)(2.3400,0.43742)(2.4000,0.66957)(2.4200,0.73592)(2.4350,0.77799)(2.4550,0.82197)(2.4700,0.84498)(2.4850,0.85895)(2.5000,0.86364)(2.5150,0.85895)(2.5250,0.85066)(2.5350,0.83830)(2.5500,0.81236)(2.5700,0.76478)(2.5850,0.72035)(2.6050,0.65146)(2.6550,0.45634)(2.6750,0.38414)(2.7000,0.30977)(2.7250,0.25132)(2.7400,0.22224)(2.7600,0.18910)(2.7750,0.16780)(2.7950,0.14336)(2.8150,0.12271)(2.8350,0.10522)(2.8550,0.09036)(2.8800,0.07484)(2.9050,0.06211)(2.9350,0.04976)(2.9650,0.03995)(3.0000,0.03099)(3.0750,0.01811)(3.1700,0.00927)(3.2800,0.00432)(3.4300,0.00155)(4.0500,0.00002)}}%


==> data/images_sketch/Lz4_err.tex <==
% generated by gen_images_sketch.py: Lz/Lx=4, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(0.0000,0.07204)(0.2400,0.06414)(0.5000,0.06150)(0.7600,0.06414)(1.0000,0.07204)}}%


==> data/images_sketch/Lz4_free.tex <==
% generated by gen_images_sketch.py: Lz/Lx=4, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.00446)(-1.6450,0.00915)(-1.3200,0.01646)(-1.0500,0.02711)(-0.8250,0.04148)(-0.6300,0.06058)(-0.5400,0.07244)(-0.4600,0.08514)(-0.3850,0.09931)(-0.3150,0.11496)(-0.2500,0.13205)(-0.1850,0.15212)(-0.1300,0.17194)(-0.0750,0.19491)(-0.0250,0.21911)(0.0200,0.24415)(0.0650,0.27294)(0.1050,0.30235)(0.1450,0.33616)(0.1800,0.37017)(0.2100,0.40336)(0.2400,0.44113)(0.2650,0.47688)(0.2900,0.51743)(0.3250,0.58460)(0.4000,0.75318)(0.4300,0.80745)(0.4500,0.83450)(0.4650,0.84924)(0.4850,0.86097)(0.5000,0.86364)(0.5150,0.86097)(0.5300,0.85304)(0.5450,0.83996)(0.5650,0.81497)(0.5800,0.79103)(0.6000,0.75318)(0.6750,0.58460)(0.6950,0.54454)(0.7150,0.50888)(0.7450,0.46206)(0.7750,0.42161)(0.8100,0.38078)(0.8500,0.34074)(0.8950,0.30235)(0.9400,0.26953)(0.9950,0.23542)(1.0500,0.20658)(1.1100,0.17989)(1.1750,0.15551)(1.2450,0.13348)(1.3150,0.11496)(1.3900,0.09829)(1.4750,0.08258)(1.5650,0.06891)(1.6650,0.05656)(1.7700,0.04611)(1.8850,0.03700)(2.1500,0.02251)(2.4550,0.01288)(2.8400,0.00646)(3.3400,0.00269)(4.0500,0.00079)}}%


==> data/images_sketch/Lz4_imgm1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=4, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.20658)(-1.9750,0.24715)(-1.9400,0.26953)(-1.9050,0.29462)(-1.8700,0.32290)(-1.8400,0.35018)(-1.8100,0.38078)(-1.7850,0.40932)(-1.7400,0.46938)(-1.7000,0.53525)(-1.6700,0.59536)(-1.6050,0.74282)(-1.5850,0.78216)(-1.5700,0.80745)(-1.5500,0.83450)(-1.5350,0.84924)(-1.5150,0.86097)(-1.5000,0.86364)(-1.4850,0.86097)(-1.4650,0.84924)(-1.4450,0.82850)(-1.4250,0.79947)(-1.4100,0.77287)(-1.3900,0.73216)(-1.3350,0.60638)(-1.3100,0.55411)(-1.2800,0.50056)(-1.2500,0.45491)(-1.2150,0.40932)(-1.1800,0.37017)(-1.1400,0.33166)(-1.1000,0.29845)(-1.0450,0.25963)(-0.9850,0.22438)(-0.9200,0.19268)(-0.8450,0.16257)(-0.7700,0.13788)(-0.6850,0.11496)(-0.5900,0.09432)(-0.4900,0.07694)(-0.3900,0.06302)(-0.2850,0.05130)(-0.1700,0.04109)(-0.0400,0.03210)(0.2550,0.01854)(0.6250,0.00948)(1.0550,0.00442)(1.6400,0.00160)(4.0500,0.00003)}}%


==> data/images_sketch/Lz4_imgp1.tex <==
% generated by gen_images_sketch.py: Lz/Lx=4, x/Lx, y = value/1.1*0.95
\def\sketchcurve{plot coordinates {(-2.0500,0.00015)(-0.2750,0.00301)(0.2150,0.00713)(0.5900,0.01397)(0.9100,0.02516)(1.0500,0.03271)(1.1750,0.04148)(1.2900,0.05180)(1.3950,0.06365)(1.4900,0.07694)(1.5800,0.09240)(1.6700,0.11139)(1.7500,0.13205)(1.8250,0.15551)(1.8950,0.18195)(1.9600,0.21148)(2.0200,0.24415)(2.0750,0.27993)(2.1250,0.31865)(2.1650,0.35503)(2.2050,0.39754)(2.2400,0.44113)(2.2750,0.49246)(2.3150,0.56397)(2.3950,0.74282)(2.4150,0.78216)(2.4350,0.81497)(2.4550,0.83996)(2.4700,0.85304)(2.4850,0.86097)(2.5000,0.86364)(2.5150,0.86097)(2.5350,0.84924)(2.5550,0.82850)(2.5750,0.79947)(2.6050,0.74282)(2.6700,0.59536)(2.6950,0.54454)(2.7350,0.47688)(2.7750,0.42161)(2.8250,0.36502)(2.8800,0.31446)(2.9400,0.26953)(3.0100,0.22708)(3.0500,0.20658)(3.0950,0.18615)(3.1400,0.16812)(3.1900,0.15045)(3.2950,0.11994)(3.4150,0.09335)(3.5450,0.07172)(3.6950,0.05333)(3.8600,0.03880)(4.0500,0.02711)}}%

